Mitigating the source-side channel vulnerability by characterization of photon statistics

Quantum key distribution (QKD) theoretically offers unconditional security. Unfortunately, the gap between theory and practice threatens side-channel attacks on practical QKD systems. Many well-known QKD protocols use weak coherent laser pulses to encode the quantum information. These sources differ from ideal single photon sources and follow Poisson statistics. Many protocols, such as decoy state and coincidence detection protocols, rely on monitoring the photon statistics to detect any information leakage. The accurate measurement and characterization of photon statistics enable the detection of adversarial attacks and the estimation of secure key rates, strengthening the overall security of the QKD system. We have rigorously characterized our source to estimate the mean photon number employing multiple detectors for comparison against measurements made with a single detector. Furthermore, we have also studied intensity fluctuations to help identify and mitigate any potential information leakage due to state preparation flaws. We aim to bridge the gap between theory and practice to achieve information-theoretic security.

==> comments.tex <==

\newpage
\section{Points to be addressed}
\begin{itemize}
    \item \textbf{Tanya}
    \begin{itemize}
    \item One of the four lasers shows a higher slope for the difference with $\mu$. Why? Due to ill working of laser? Due to high fluctuations? Should we report this difference? Or should I just remove it?
    \item check the equations, in theory.
    \item Other methods \cite{Dynes2018}based on the calculation of correlation function assume low detection efficiencies.
    \end{itemize}

    \item \textbf{Pooja}
    \begin{itemize}

    
    \item add references in para 3 intro, add excelitas data-sheet in references
    \item Make in flow and add some explanation in the results
    \item this experiment was done before? In conclusion or discuss
    \item \textcolor{green}{If you have mentioned the abbreviation above, then do not need to write the full form again}
    \end{itemize}    
    
    \item \textbf{Ayan} 
    \begin{itemize}
        \item If the source is known to be Poisson, then also it will be necessary to calculate $\mu$ using four detectors?
        \item What is basis of calculating $I(A:E)_{I}$? I though that there will be only one mutual information i.e due to the miscalculation in $\mu$ from one detector rather that using 4, which will lead to side channel as we are predicting the wrong $\mu$.
        \item I think it will be good if we can add the fluctuation in the result section otherwise it is small. Or we may have to elaborate the result section. 
    \end{itemize}
    \item \textbf{Jayanth} 
    \begin{itemize}
        \item \textcolor{green}{Accurate estimation vs Precise estimation. They both have different meanings and it is important that it be consistent. I have noticed that both terms are in use.}
        \item In Sec 2. Subsec C., in Rigorous characterisation, there is no definition of branching efficiencies. Further, a small diagram could be included which will help make the definitions clearer.
        \item The picture of the experimental setup must be bigger.
        \item In Sec 2. Subsec D., there is only a sentence mentioning the information gained by Eve. More description may be required : more about attack 2 sentences
        \item I feel that in the abstract sentences are getting repetitive. A slight revision may be needed. 
    \end{itemize}   
\end{itemize}  
